Continuously Generalized Ordinal Regression for Linear and Deep Models

Ordinal regression is a classification task where classes have an order and prediction error increases the further the predicted class is from the true class. The standard approach for modeling ordinal data involves fitting parallel separating hyperplanes that optimize a certain loss function. This assumption offers sample efficient learning via inductive bias, but is often too restrictive in real-world datasets where features may have varying effects across different categories. Allowing class-specific hyperplane slopes creates generalized logistic ordinal regression, increasing the flexibility of the model at a cost to sample efficiency. We explore an extension of the generalized model to the all-thresholds logistic loss and propose a regularization approach that interpolates between these two extremes. Our method, which we term continuously generalized ordinal logistic, significantly outperforms the standard ordinal logistic model over a thorough set of ordinal regression benchmark datasets. We further extend this method to deep learning and show that it achieves competitive or lower prediction error compared to previous models over a range of datasets and modalities. Furthermore, two primary alternative models for deep learning ordinal regression are shown to be special cases of our framework.

==> bench_table.tex <==

\begin{tabular}{llrrr}
\toprule
     Dataset    & Model   &  MAE &  MSE &  Accuracy \\
\midrule
\multirow{3}{*}{ERA} & OL &     1.216 &     2.539 &     0.251 \\
                & GOL &     1.205 &     2.489 &     0.245 \\
                & coGOL &     \textbf{1.200} &     \textbf{2.523} &     \textbf{0.259} \\
\cline{1-5}
\multirow{3}{*}{ESL} & OL &     0.307 &     0.346 &     0.710 \\
                & GOL &     0.314 &     0.349 &     0.704 \\
                & coGOL &     \textbf{0.299} &     \textbf{0.332} &     \textbf{0.717} \\
\cline{1-5}
\multirow{3}{*}{LEV} & OL &     \textbf{0.413} &     \textbf{0.485} &     \textbf{0.619} \\
                & GOL &     0.435 &     0.509 &     0.598 \\
                & coGOL &     0.418 &     0.491 &     0.615 \\
\cline{1-5}
\multirow{3}{*}{SWD} & OL &     0.449 &     0.484 &     0.569 \\
                & GOL &     0.436 &     \textbf{0.464} &     0.578 \\
                & coGOL &     \textbf{0.433} &     \textbf{0.464} &     \textbf{0.582} \\
\cline{1-5}
\multirow{3}{*}{automobile} & OL &     0.453 &     0.594 &     0.607 \\
                & GOL &     \textbf{0.350} &     \textbf{0.472} &     0.709 \\
                & coGOL &     0.366 &     0.533 &     \textbf{0.710} \\
\cline{1-5}
\multirow{3}{*}{balance-scale} & OL &     \textbf{0.107} &     \textbf{0.131} &     \textbf{0.906} \\
                & GOL &     0.108 &     0.133 &     0.905 \\
                & coGOL &     \textbf{0.107} &     0.132 &     0.905 \\
\cline{1-5}
\multirow{3}{*}{bondrate} & OL &     0.556 &     0.747 &     0.540 \\
                & GOL &     0.518 &     0.718 &     0.582 \\
                & coGOL &     \textbf{0.502} &     \textbf{0.676} &     \textbf{0.584} \\
\cline{1-5}
\multirow{3}{*}{car} & OL &     0.091 &     0.096 &     0.912 \\
                & GOL &     0.102 &     0.120 &     0.907 \\
                & coGOL &     \textbf{0.074} &     \textbf{0.080} &     \textbf{0.929} \\
\cline{1-5}
\multirow{3}{*}{contact-lenses} & OL &     0.394 &     \textbf{0.483} &     0.650 \\
                & GOL &     \textbf{0.372} &     0.517 &     \textbf{0.700} \\
                & coGOL &     0.411 &     0.611 &     0.689 \\
\cline{1-5}
\multirow{3}{*}{eucalyptus} & OL &     0.389 &     \textbf{0.449} &     0.639 \\
                & GOL &     0.414 &     0.525 &     0.631 \\
                & coGOL &     \textbf{0.386} &     0.456 &     \textbf{0.645} \\
\cline{1-5}
\multirow{3}{*}{newthyroid} & OL &     0.052 &     0.052 &     0.948 \\
                & GOL &     0.075 &     0.075 &     0.925 \\
                & coGOL &     \textbf{0.043} &     \textbf{0.043} &     \textbf{0.957} \\
\cline{1-5}
\multirow{3}{*}{pasture} & OL &     0.341 &     0.341 &     0.659 \\
                & GOL &     \textbf{0.307} &     \textbf{0.307} &     \textbf{0.693} \\
                & coGOL &     0.333 &     0.333 &     0.667 \\
\cline{1-5}
\multirow{3}{*}{squash-stored} & OL &     0.356 &     \textbf{0.367} &     0.649 \\
                & GOL &     0.377 &     0.433 &     0.651 \\
                & coGOL &     \textbf{0.354} &     0.395 &     \textbf{0.667} \\
\cline{1-5}
\multirow{3}{*}{squash-unstored} & OL &     \textbf{0.277} &     \textbf{0.277} &     0.723 \\
                & GOL &     \textbf{0.277} &     0.292 &     0.731 \\
                & coGOL &     \textbf{0.277} &     0.303 &     \textbf{0.736} \\
\cline{1-5}
\multirow{3}{*}{tae} & OL &     0.623 &     0.798 &     0.465 \\
                & GOL &     \textbf{0.579} &     0.779 &     \textbf{0.521} \\
                & coGOL &     0.581 &     \textbf{0.770} &     0.514 \\
\cline{1-5}
\multirow{3}{*}{toy} & OL &     0.994 &     1.606 &     0.281 \\
                & GOL &     0.908 &     \textbf{1.328} &     0.286 \\
                & coGOL &    \textbf{0.904} &     \textbf{1.328} &     \textbf{0.289} \\
\cline{1-5}
\multirow{3}{*}{winequality-red} & OL &     0.440 &     0.509 &     0.593 \\
                & GOL &     \textbf{0.433} &     \textbf{0.504} &     \textbf{0.600} \\
                & coGOL &     0.436 &     0.506 &     0.598 \\
\bottomrule
\end{tabular}

% \end{table}



==> bench_table_joint.tex <==
% \begin{table}[]
\begin{tabular}{@{}llcccccc@{}}
\toprule
                                       &                               & \multicolumn{3}{c}{Linear}                       & \multicolumn{3}{c}{RBF}                          \\ \cmidrule(l){3-5} \cmidrule(l){6-8}
\multicolumn{1}{c}{Dataset}            & \multicolumn{1}{c}{Model} & MAE            & MSE            & Acc            & MAE            & MSE            & Acc            \\ \midrule
\multirow{3}{*}{{\ul ERA}}             & OL                            & 1.216          & 2.539          & 0.251          & 1.220          & 2.536          & 0.245          \\
                                       & GOL                           & 1.205          & 2.489          & 0.245          & 1.310          & 2.913          & 0.237          \\
                                       & coGOL                         & \textbf{1.200} & \textbf{2.523} & \textbf{0.259} & 1.218          & 2.604          & 0.263          \\ \midrule
\multirow{3}{*}{ESL*}                  & OL                            & 0.307          & 0.346          & 0.710          & \textbf{0.294} & \textbf{0.324} & \textbf{0.719} \\
                                       & GOL                           & 0.314          & 0.349          & 0.704          & 0.308          & 0.338          & 0.705          \\
                                       & coGOL                         & \textbf{0.299} & \textbf{0.332} & \textbf{0.717} & \textit{0.300} & \textit{0.327} & \textit{0.712} \\ \midrule
\multirow{3}{*}{LEV*}                  & OL                            & \textbf{0.413} & \textbf{0.485} & \textbf{0.619} & 0.416          & 0.495          & 0.621          \\
                                       & GOL                           & 0.435          & 0.509          & 0.598          & \textit{0.406} & \textit{0.484} & \textit{0.629} \\
                                       & coGOL                         & 0.299          & 0.332          & 0.717          & \textbf{0.401} & \textbf{0.476} & \textbf{0.633} \\ \midrule
\multirow{3}{*}{{\ul SWD}}             & OL                            & 0.449          & 0.484          & 0.569          & 0.441          & 0.475          & 0.576          \\
                                       & GOL                           & 0.436          & \textbf{0.464} & 0.578          & 0.434          & 0.465          & 0.581          \\
                                       & coGOL                         & \textbf{0.433} & \textbf{0.464} & \textbf{0.582} & 0.437          & 0.469          & 0.579          \\ \midrule
\multirow{3}{*}{{\ul automobile}}      & OL                            & 0.453          & 0.594          & 0.607          & 0.625          & 0.905          & 0.500          \\
                                       & GOL                           & \textbf{0.350} & \textbf{0.472} & 0.709          & 0.431          & 0.624          & 0.659          \\
                                       & coGOL                         & 0.366          & 0.533          & \textbf{0.710} & 0.412          & 0.618          & 0.684          \\ \midrule
\multirow{3}{*}{balance-scale*}        & OL                            & \textbf{0.107} & \textbf{0.131} & \textbf{0.906} & \textbf{0.014} & \textbf{0.014} & \textbf{0.986} \\
                                       & GOL                           & 0.108          & 0.133          & 0.905          & 0.023          & 0.023          & 0.977          \\
                                       & coGOL                         & \textbf{0.107} & 0.132          & 0.905          & \textit{0.020} & \textit{0.020} & \textit{0.980} \\ \midrule
\multirow{3}{*}{{\ul bondrate}}        & OL                            & 0.556          & 0.747          & 0.540          & 0.611          & 1.091          & 0.579          \\
                                       & GOL                           & 0.518          & 0.718          & 0.582          & 0.664          & 1.197          & 0.541          \\
                                       & coGOL                         & \textbf{0.502} & \textbf{0.676} & \textbf{0.584} & 0.640          & 1.163          & 0.563          \\ \midrule
\multirow{3}{*}{{\ul car}}             & OL                            & 0.091          & 0.096          & 0.912          & 0.418          & 0.628          & 0.667          \\
                                       & GOL                           & 0.102          & 0.120          & 0.907          & 0.363          & 0.541          & 0.709          \\
                                       & coGOL                         & \textbf{0.074} & \textbf{0.080} & \textbf{0.929} & 0.362          & 0.539          & 0.709          \\ \midrule
\multirow{3}{*}{{\ul contact-lenses}}  & OL                            & 0.394          & \textbf{0.483} & 0.650          & 0.676          & 0.990          & 0.480          \\
                                       & GOL                           & \textbf{0.372} & 0.517          & \textbf{0.700} & 0.657          & 0.971          & 0.500          \\
                                       & coGOL                         & 0.411          & 0.611          & 0.689          & 0.686          & 1.039          & 0.490          \\ \midrule
\multirow{3}{*}{{\ul eucalyptus}}      & OL                            & 0.389          & \textbf{0.449} & 0.639          & 0.511          & 0.700          & 0.567          \\
                                       & GOL                           & 0.414          & 0.525          & 0.631          & 0.511          & 0.747          & 0.579          \\
                                       & coGOL                         & \textbf{0.386} & 0.456          & \textbf{0.645} & 0.474          & 0.660          & 0.597          \\ \midrule
\multirow{3}{*}{{\ul newthyroid}}      & OL                            & 0.052          & 0.052          & 0.948          & 0.047          & 0.049          & 0.954          \\
                                       & GOL                           & 0.075          & 0.075          & 0.925          & 0.047          & 0.049          & 0.954          \\
                                       & coGOL                         & \textbf{0.043} & \textbf{0.043} & \textbf{0.957} & 0.048          & 0.050          & 0.953          \\ \midrule
\multirow{3}{*}{{\ul pasture}}         & OL                            & 0.341          & 0.341          & 0.659          & 0.464          & 0.503          & 0.556          \\
                                       & GOL                           & \textbf{0.307} & \textbf{0.307} & \textbf{0.693} & 0.471          & 0.549          & 0.569          \\
                                       & coGOL                         & 0.333          & 0.333          & 0.667          & 0.477          & 0.542          & 0.556          \\ \midrule
\multirow{3}{*}{{\ul squash-stored}}   & OL                            & 0.356          & \textbf{0.367} & 0.649          & 0.506          & 0.551          & 0.516          \\
                                       & GOL                           & 0.377          & 0.433          & 0.651          & 0.481          & 0.538          & 0.548          \\
                                       & coGOL                         & \textbf{0.354} & 0.395          & \textbf{0.677} & 0.471          & 0.503          & 0.545          \\ \midrule
\multirow{3}{*}{{\ul squash-unstored}} & OL                            & \textbf{0.277} & \textbf{0.277} & 0.723          & 0.335          & 0.335          & 0.665          \\
                                       & GOL                           & \textbf{0.277} & 0.292          & 0.731          & 0.344          & 0.344          & 0.656          \\
                                       & coGOL                         & \textbf{0.277} & 0.303          & \textbf{0.736} & 0.348          & 0.348          & 0.652          \\ \midrule
\multirow{3}{*}{{\ul tae}}             & OL                            & 0.623          & 0.798          & 0.465          & 0.588          & 0.772          & 0.504          \\
                                       & GOL                           & \textbf{0.579} & 0.779          & \textbf{0.521} & 0.582          & 0.774          & 0.514          \\
                                       & coGOL                         & 0.581          & \textbf{0.770} & 0.514          & 0.597          & 0.803          & 0.505          \\ \midrule
\multirow{3}{*}{toy*}                  & OL                            & 0.994          & 1.606          & 0.281          & \textbf{0.023} & \textbf{0.023} & \textbf{0.977} \\
                                       & GOL                           & 0.908          & \textbf{1.328} & 0.286          & 0.053          & 0.053          & 0.947          \\
                                       & coGOL                         & \textbf{0.904} & \textbf{1.328} & \textbf{0.289} & \textit{0.049} & \textit{0.049} & \textit{0.951} \\ \midrule
\multirow{3}{*}{winequality-red*}      & OL                            & 0.440          & 0.509          & 0.593          & \textit{0.435} & \textit{0.540} & \textbf{0.611} \\
                                       & GOL                           & \textbf{0.433} & \textbf{0.504} & \textbf{0.600} & 0.446          & 0.556          & 0.605          \\
                                       & coGOL                         & 0.436          & 0.506          & 0.598          & \textbf{0.433} & \textbf{0.524} & \textit{0.608} \\ \bottomrule
\end{tabular}
% \end{table}

==> bench_table_joint_wide.tex <==
\begin{tabular}{@{}llcccccclcccccc@{}}
\toprule
                                      &                           & \multicolumn{3}{c}{Linear}                       & \multicolumn{3}{c}{RBF}                          &                                        & \multicolumn{3}{c}{Linear}                       & \multicolumn{3}{c}{RBF}                          \\  \cmidrule(lr){3-5}\cmidrule(lr){6-8} \cmidrule(l){10-12} \cmidrule(l){13-15} 
\multicolumn{1}{c}{Dataset}           & \multicolumn{1}{c}{Model} & MAE            & MSE            & Acc            & MAE            & MSE            & Acc            & \multicolumn{1}{c}{Dataset}            & MAE            & MSE            & Acc            & MAE            & MSE            & Acc            \\ \midrule
\multirow{3}{*}{{\ul ERA}}            & OL                        & 1.216          & 2.539          & 0.251          & 1.212          & 2.512          & 0.252          & \multirow{3}{*}{{\ul eucalyptus}}      & 0.389          & \textbf{0.449} & 0.639          & 0.516          & 0.712          & 0.560          \\
                                      & GOL                       & 1.205          & 2.489          & 0.245          & 1.224          & 2.788          & 0.240          &                                        & 0.414          & 0.525          & 0.631          & 0.500          & 0.723          & 0.582          \\
                                      & coGOL                     & \textbf{1.200} & \textbf{2.523} & \textbf{0.259} & 1.216          & 2.584          & 0.264          &                                        & \textbf{0.386} & 0.456          & \textbf{0.645} & 0.462          & 0.603          & 0.598          \\ \midrule
\multirow{3}{*}{\ul ESL}                 & OL                        & 0.307          & 0.346          & 0.710          & 0.303 & 0.328 & 0.713 & \multirow{3}{*}{{newthyroid*}}      & 0.052          & 0.052          & 0.948          & \textbf{0.037}          & \textbf{0.037}          & \textbf{0.963}          \\
                                      & GOL                       & 0.314          & 0.349          & 0.704          & 0.320          & 0.344          & 0.689          &                                        & 0.075          & 0.075          & 0.925          & \textbf{0.037}          & \textbf{0.037 }         & \textbf{0.963}          \\
                                      & coGOL                     & \textbf{0.299} & \textbf{0.332} & \textbf{0.717} & 0.311 & 0.336 & 0.697 &                                        & \textbf{0.043} & \textbf{0.043} & \textbf{0.957} & \textbf{0.037}          & \textbf{0.037}          & \textbf{0.963}          \\ \midrule
\multirow{3}{*}{LEV*}                 & OL                        & \textbf{0.413} & \textbf{0.485} & \textbf{0.619} & 0.414          & 0.496          & 0.620          & \multirow{3}{*}{{\ul pasture}}         & 0.341          & 0.341          & 0.659          & 0.444          & 0.444          & 0.556          \\
                                      & GOL                       & 0.435          & 0.509          & 0.598          & \textit{0.410} & \textit{0.492} & \textbf{0.630} &                                        & \textbf{0.307} & \textbf{0.307} & \textbf{0.693} & 0.444          & 0.444          & 0.556          \\
                                      & coGOL                     & 0.418          &     0.491      &     0.615          & \textbf{0.406} & \textbf{0.482} & \textit{0.628} &                                        & 0.333          & 0.333          & 0.667          & 0.444          & 0.444          & 0.556          \\ \midrule
\multirow{3}{*}{{\ul SWD}}            & OL                        & 0.449          & 0.484          & 0.569          & 0.436          & 0.474          & 0.582          & \multirow{3}{*}{{\ul squash-stored}}   & 0.356          & \textbf{0.367} & 0.649          & 0.462          & 0.462          & 0.538          \\
                                      & GOL                       & 0.436          & \textbf{0.464} & 0.578          & 0.438          & 0.472          & 0.580          &                                        & 0.377          & 0.433          & 0.651          & 0.462          & 0.538          & 0.615          \\
                                      & coGOL                     & \textbf{0.433} & \textbf{0.464} & \textbf{0.582} & 0.438          & 0.470          & 0.580          &                                        & \textbf{0.354} & 0.395          & \textbf{0.677} & 0.385          & 0.423          & 0.615          \\ \midrule
\multirow{3}{*}{{\ul automobile}}     & OL                        & 0.453          & 0.594          & 0.607          & 0.596          & 0.808          & 0.500          & \multirow{3}{*}{{\ul squash-unstored}} & \textbf{0.277} & \textbf{0.277} & 0.723          & 0.308          & 0.308          & 0.692          \\
                                      & GOL                       & \textbf{0.350} & \textbf{0.472} & 0.709          & 0.404          & 0.558          & 0.673          &                                        & \textbf{0.277} & 0.292          & 0.731          & 0.308          & 0.308          & 0.692          \\
                                      & coGOL                     & 0.366          & 0.533          & \textbf{0.710} & 0.404          & 0.615          & 0.673          &                                        & \textbf{0.277} & 0.303          & \textbf{0.736}          & 0.308          & 0.308          & 0.692          \\ \midrule
\multirow{3}{*}{balance-scale*}       & OL                        & \textbf{0.107} & \textbf{0.131} & \textbf{0.906} & \textbf{0.013} & \textbf{0.013} & \textbf{0.987} & \multirow{3}{*}{{tae*}}             & 0.623          & 0.798          & 0.465          & \textbf{0.553}          & \textbf{0.724}          & 0.500          \\
                                      & GOL                       & 0.108          & 0.133          & 0.905          & 0.019          & 0.019          & 0.981          &                                        & \textbf{0.579} & 0.779          & \textbf{0.521} & 0.579          & \textit{0.776 }         & \textit{0.513}          \\
                                      & coGOL                     & \textbf{0.107} & 0.132          & 0.905          & \textit{0.016} & \textit{0.016} & \textit{0.984} &                                        & 0.581          & \textbf{0.770} & 0.514          & \textit{0.566}          & \textit{0.776}          & \textbf{0.526}          \\ \midrule
\multirow{3}{*}{{\ul bondrate}}       & OL                        & 0.556          & 0.747          & 0.540          & 0.600          & 1.133          & 0.600          & \multirow{3}{*}{{toy*}}            & 0.994          & 1.606          & 0.281          & \textbf{0.020} & \textbf{0.020} & \textbf{0.980} \\
                                      & GOL                       & 0.518          & 0.718          & 0.582          & 0.667          & 1.200          & 0.533          &                                        & 0.908          & \textbf{1.328} & 0.286          & 0.053          & 0.053          & 0.947          \\
                                      & coGOL                     & \textbf{0.502} & \textbf{0.676} & \textbf{0.584} & 0.633          & 1.133          & 0.567          &                                        & \textbf{0.904} & \textbf{1.328} & \textbf{0.289} & \textit{0.040}          & \textit{0.040}          & \textit{0.960}          \\ \midrule
\multirow{3}{*}{{\ul car}}            & OL                        & 0.091          & 0.096          & 0.912          & 0.412          & 0.587          & 0.676          & \multirow{3}{*}{winequality-red*}      & 0.440          & 0.509          & 0.593          & \textit{0.435}          & \textit{0.540}          & \textbf{0.611}          \\
                                      & GOL                       & 0.102          & 0.120          & 0.907          & 0.339          & 0.426          & 0.701          &                                        & \textbf{0.433} & \textbf{0.504} & \textbf{0.600} & 0.446          & 0.556          & 0.605 \\
                                      & coGOL                     & \textbf{0.074} & \textbf{0.080} & \textbf{0.929} & 0.325          & 0.411          & 0.712          &                                        & 0.436          & 0.506          & 0.598          & \textbf{0.433} & \textbf{0.524} & \textit{0.608}          \\ \midrule
\multirow{3}{*}{{\ul contact-lenses}} & OL                        & 0.394          & \textbf{0.483} & 0.650          & 0.667          & 0.917          & 0.500          & \multirow{3}{*}{}                      &                &                &                &                &                &                \\
                                      & GOL                       & \textbf{0.372} & 0.517          & \textbf{0.700} & 0.583          & 0.833          & 0.500          &                                        &                &                &                &                &                &                \\
                                      & coGOL                     & 0.411          & 0.611          & 0.689          & 0.667          & 0.917          & 0.500          &                                        &                &                &                &                &                &                \\ \bottomrule
\end{tabular}

==> data_info_table.tex <==
\begin{table}[ht]
\centering
\label{tab:info}
\caption{Characteristics of the 17 benchmark datasets for ordinal regression. These are datasets with real ordinal targets, unlike many benchmark datasets which discretize a regression target into ordinal classes.}
\begin{tabular}{llll}
\toprule
Dataset & Samples & Features & Classes \\
\midrule
ERA & 1000 & 4 & 9 \\
ESL & 488 & 4 & 9 \\
LEV & 1000 & 4 & 5 \\
SWD & 1000 & 10 & 4 \\
automobile & 205 & 71 & 6 \\
balance-scale & 625 & 4 & 3 \\
bondrate & 57 & 37 & 5 \\
car & 1728 & 21 & 4 \\
contact-lenses & 24 & 6 & 3 \\
eucalyptus & 736 & 91 & 5 \\
newthyroid & 215 & 5 & 3 \\
pasture & 36 & 25 & 3 \\
squash-stored & 52 & 51 & 3 \\
squash-unstored & 52 & 52 & 3 \\
tae & 151 & 54 & 3 \\
toy & 300 & 2 & 5 \\
winequality-red & 1599 & 11 & 6 \\
\bottomrule
\end{tabular}
\end{table}

==> fused_bench_table_NEW.tex <==
\begin{tabular}{llrrr}
\toprule
                &       &  test\_mae &  test\_mse &  test\_1-0 \\
dataset & model &           &           &           \\
\midrule
\multirow{3}{*}{ERA} & OL &     1.210 &     2.533 &     0.256 \\
                & GOL &     1.192 &     2.509 &     0.264 \\
                & coGOL &     1.193 &     2.514 &     0.264 \\
\cline{1-5}
\multirow{3}{*}{ESL} & OL &     0.310 &     0.345 &     0.705 \\
                & GOL &     0.309 &     0.340 &     0.706 \\
                & coGOL &     0.293 &     0.324 &     0.722 \\
\cline{1-5}
\multirow{3}{*}{LEV} & OL &     0.416 &     0.490 &     0.618 \\
                & GOL &     0.434 &     0.509 &     0.601 \\
                & coGOL &     0.421 &     0.494 &     0.613 \\
\cline{1-5}
\multirow{3}{*}{SWD} & OL &     0.448 &     0.484 &     0.570 \\
                & GOL &     0.435 &     0.464 &     0.579 \\
                & coGOL &     0.433 &     0.464 &     0.582 \\
\cline{1-5}
\multirow{3}{*}{automobile} & OL &     0.454 &     0.601 &     0.607 \\
                & GOL &     0.369 &     0.513 &     0.696 \\
                & coGOL &     0.379 &     0.590 &     0.714 \\
\cline{1-5}
\multirow{3}{*}{balance-scale} & OL &     0.107 &     0.130 &     0.905 \\
                & GOL &     0.107 &     0.131 &     0.905 \\
                & coGOL &     0.107 &     0.131 &     0.905 \\
\cline{1-5}
\multirow{3}{*}{bondrate} & OL &     0.549 &     0.767 &     0.556 \\
                & GOL &     0.564 &     0.818 &     0.556 \\
                & coGOL &     0.536 &     0.744 &     0.562 \\
\cline{1-5}
\multirow{3}{*}{car} & OL &     0.082 &     0.083 &     0.919 \\
                & GOL &     0.073 &     0.077 &     0.930 \\
                & coGOL &     0.073 &     0.078 &     0.930 \\
\cline{1-5}
\multirow{3}{*}{contact-lenses} & OL &     0.428 &     0.601 &     0.659 \\
                & GOL &     0.384 &     0.572 &     0.710 \\
                & coGOL &     0.406 &     0.623 &     0.703 \\
\cline{1-5}
\multirow{3}{*}{eucalyptus} & OL &     0.396 &     0.457 &     0.634 \\
                & GOL &     0.404 &     0.502 &     0.636 \\
                & coGOL &     0.398 &     0.486 &     0.641 \\
\cline{1-5}
\multirow{3}{*}{newthyroid} & OL &     0.029 &     0.029 &     0.971 \\
                & GOL &     0.033 &     0.033 &     0.967 \\
                & coGOL &     0.030 &     0.030 &     0.970 \\
\cline{1-5}
\multirow{3}{*}{pasture} & OL &     0.333 &     0.333 &     0.667 \\
                & GOL &     0.283 &     0.283 &     0.717 \\
                & coGOL &     0.328 &     0.328 &     0.672 \\
\cline{1-5}
\multirow{3}{*}{squash-stored} & OL &     0.416 &     0.437 &     0.594 \\
                & GOL &     0.381 &     0.430 &     0.643 \\
                & coGOL &     0.378 &     0.413 &     0.640 \\
\cline{1-5}
\multirow{3}{*}{squash-unstored} & OL &     0.289 &     0.289 &     0.711 \\
                & GOL &     0.282 &     0.297 &     0.725 \\
                & coGOL &     0.275 &     0.289 &     0.733 \\
\cline{1-5}
\multirow{3}{*}{tae} & OL &     0.614 &     0.752 &     0.455 \\
                & GOL &     0.575 &     0.761 &     0.518 \\
                & coGOL &     0.580 &     0.741 &     0.500 \\
\cline{1-5}
\multirow{3}{*}{toy} & OL &     0.953 &     1.464 &     0.287 \\
                & GOL &     0.899 &     1.325 &     0.294 \\
                & coGOL &     0.898 &     1.324 &     0.295 \\
\cline{1-5}
\multirow{3}{*}{winequality-red} & OL &     0.443 &     0.515 &     0.592 \\
                & GOL &     0.436 &     0.511 &     0.600 \\
                & coGOL &     0.438 &     0.516 &     0.598 \\
\bottomrule
\end{tabular}

==> kernel_bench_table.tex <==
% \begin{tabular}{llrrr}
% \toprule
%                 &             &  test\_mae &  test\_mse &  test\_1-0 \\
% dataset & model &           &           &           \\
% \midrule
% \multirow{3}{*}{ERA} & OL (rbf) &     1.239 &     2.591 &     0.237 \\
%                 & GOL (rbf) &     1.257 &     2.740 &     0.245 \\
%                 & coGOL (rbf) &     1.253 &     2.744 &     0.253 \\
% \cline{1-5}
% \multirow{3}{*}{ESL} & OL (rbf) &     0.463 &     0.666 &     0.601 \\
%                 & GOL (rbf) &     0.373 &     0.420 &     0.650 \\
%                 & coGOL (rbf) &     0.368 &     0.411 &     0.654 \\
% \cline{1-5}
% \multirow{3}{*}{LEV} & OL (rbf) &     0.416 &     0.489 &     0.618 \\
%                 & GOL (rbf) &     0.400 &     0.476 &     0.633 \\
%                 & coGOL (rbf) &     0.403 &     0.480 &     0.631 \\
% \cline{1-5}
% \multirow{3}{*}{SWD} & OL (rbf) &     0.447 &     0.483 &     0.571 \\
%                 & GOL (rbf) &     0.438 &     0.473 &     0.579 \\
%                 & coGOL (rbf) &     0.445 &     0.480 &     0.573 \\
% \cline{1-5}
% \multirow{3}{*}{automobile} & OL (rbf) &     0.640 &     0.920 &     0.488 \\
%                 & GOL (rbf) &     0.540 &     0.815 &     0.589 \\
%                 & coGOL (rbf) &     0.532 &     0.816 &     0.599 \\
% \cline{1-5}
% \multirow{3}{*}{balance-scale} & OL (rbf) &     0.012 &     0.012 &     0.988 \\
%                 & GOL (rbf) &     0.028 &     0.028 &     0.972 \\
%                 & coGOL (rbf) &     0.014 &     0.014 &     0.986 \\
% \cline{1-5}
% \multirow{3}{*}{bondrate} & OL (rbf) &     0.604 &     1.107 &     0.593 \\
%                 & GOL (rbf) &     0.607 &     1.096 &     0.581 \\
%                 & coGOL (rbf) &     0.607 &     1.096 &     0.581 \\
% \cline{1-5}
% \multirow{3}{*}{car} & OL (rbf) &     0.418 &     0.697 &     0.688 \\
%                 & GOL (rbf) &     0.402 &     0.673 &     0.702 \\
%                 & coGOL (rbf) &     0.403 &     0.670 &     0.699 \\
% \cline{1-5}
% \multirow{3}{*}{contact-lenses} & OL (rbf) &     0.637 &     1.010 &     0.549 \\
%                 & GOL (rbf) &     0.569 &     0.941 &     0.618 \\
%                 & coGOL (rbf) &     0.569 &     0.941 &     0.618 \\
% \cline{1-5}
% \multirow{3}{*}{eucalyptus} & OL (rbf) &     0.513 &     0.717 &     0.569 \\
%                 & GOL (rbf) &     0.614 &     0.965 &     0.520 \\
%                 & coGOL (rbf) &     0.555 &     0.816 &     0.547 \\
% \cline{1-5}
% \multirow{3}{*}{newthyroid} & OL (rbf) &     0.086 &     0.088 &     0.915 \\
%                 & GOL (rbf) &     0.070 &     0.081 &     0.936 \\
%                 & coGOL (rbf) &     0.069 &     0.082 &     0.938 \\
% \cline{1-5}
% \multirow{3}{*}{pasture} & OL (rbf) &     0.586 &     0.586 &     0.414 \\
%                 & GOL (rbf) &     0.660 &     0.673 &     0.346 \\
%                 & coGOL (rbf) &     0.667 &     0.667 &     0.333 \\
% \cline{1-5}
% \multirow{3}{*}{squash-stored} & OL (rbf) &     0.568 &     0.568 &     0.432 \\
%                 & GOL (rbf) &     0.568 &     0.568 &     0.432 \\
%                 & coGOL (rbf) &     0.568 &     0.568 &     0.432 \\
% \cline{1-5}
% \multirow{3}{*}{squash-unstored} & OL (rbf) &     0.538 &     0.538 &     0.462 \\
%                 & GOL (rbf) &     0.538 &     0.538 &     0.462 \\
%                 & coGOL (rbf) &     0.538 &     0.538 &     0.462 \\
% \cline{1-5}
% \multirow{3}{*}{tae} & OL (rbf) &     0.630 &     0.769 &     0.440 \\
%                 & GOL (rbf) &     0.655 &     0.794 &     0.415 \\
%                 & coGOL (rbf) &     0.635 &     0.780 &     0.438 \\
% \cline{1-5}
% \multirow{3}{*}{toy} & OL (rbf) &     0.022 &     0.022 &     0.978 \\
%                 & GOL (rbf) &     0.049 &     0.049 &     0.951 \\
%                 & coGOL (rbf) &     0.048 &     0.048 &     0.952 \\
% \cline{1-5}
% \multirow{3}{*}{winequality-red} & OL (rbf) &     0.429 &     0.537 &     0.619 \\
%                 & GOL (rbf) &     0.442 &     0.553 &     0.610 \\
%                 & coGOL (rbf) &     0.422 &     0.520 &     0.621 \\
% \bottomrule
% \end{tabular}


\begin{tabular}{llrrr}
\toprule
                &             &  test\_mae &  test\_mse &  test\_1-0 \\
dataset & model &           &           &           \\
\midrule
\multirow{3}{*}{ERA} & OL (rbf) &     1.212 &     2.512 &     0.252 \\
                & GOL (rbf) &     1.224 &     2.788 &     0.240 \\
                & coGOL (rbf) &     1.216 &     2.584 &     0.264 \\
\cline{1-5}
\multirow{3}{*}{ESL} & OL (rbf) &     0.303 &     0.328 &     0.713 \\
                & GOL (rbf) &     0.320 &     0.344 &     0.689 \\
                & coGOL (rbf) &     0.311 &     0.336 &     0.697 \\
\cline{1-5}
\multirow{3}{*}{LEV} & OL (rbf) &     0.414 &     0.496 &     0.620 \\
                & GOL (rbf) &     0.410 &     0.492 &     0.630 \\
                & coGOL (rbf) &     0.406 &     0.482 &     0.628 \\
\cline{1-5}
\multirow{3}{*}{SWD} & OL (rbf) &     0.436 &     0.474 &     0.582 \\
                & GOL (rbf) &     0.438 &     0.472 &     0.580 \\
                & coGOL (rbf) &     0.438 &     0.470 &     0.580 \\
\cline{1-5}
\multirow{3}{*}{automobile} & OL (rbf) &     0.596 &     0.808 &     0.500 \\
                & GOL (rbf) &     0.404 &     0.558 &     0.673 \\
                & coGOL (rbf) &     0.404 &     0.615 &     0.673 \\
\cline{1-5}
\multirow{3}{*}{balance-scale} & OL (rbf) &     0.013 &     0.013 &     0.987 \\
                & GOL (rbf) &     0.019 &     0.019 &     0.981 \\
                & coGOL (rbf) &     0.016 &     0.016 &     0.984 \\
\cline{1-5}
\multirow{3}{*}{bondrate} & OL (rbf) &     0.600 &     1.133 &     0.600 \\
                & GOL (rbf) &     0.667 &     1.200 &     0.533 \\
                & coGOL (rbf) &     0.633 &     1.133 &     0.567 \\
\cline{1-5}
\multirow{3}{*}{car} & OL (rbf) &     0.412 &     0.587 &     0.676 \\
                & GOL (rbf) &     0.339 &     0.426 &     0.701 \\
                & coGOL (rbf) &     0.325 &     0.411 &     0.712 \\
\cline{1-5}
\multirow{3}{*}{contact-lenses} & OL (rbf) &     0.667 &     0.917 &     0.500 \\
                & GOL (rbf) &     0.583 &     0.833 &     0.500 \\
                & coGOL (rbf) &     0.667 &     0.917 &     0.500 \\
\cline{1-5}
\multirow{3}{*}{eucalyptus} & OL (rbf) &     0.516 &     0.712 &     0.560 \\
                & GOL (rbf) &     0.500 &     0.723 &     0.582 \\
                & coGOL (rbf) &     0.462 &     0.603 &     0.598 \\
\cline{1-5}
\multirow{3}{*}{newthyroid} & OL (rbf) &     0.037 &     0.037 &     0.963 \\
                & GOL (rbf) &     0.037 &     0.037 &     0.963 \\
                & coGOL (rbf) &     0.037 &     0.037 &     0.963 \\
\cline{1-5}
\multirow{3}{*}{pasture} & OL (rbf) &     0.444 &     0.444 &     0.556 \\
                & GOL (rbf) &     0.444 &     0.444 &     0.556 \\
                & coGOL (rbf) &     0.444 &     0.444 &     0.556 \\
\cline{1-5}
\multirow{3}{*}{squash-stored} & OL (rbf) &     0.462 &     0.462 &     0.538 \\
                & GOL (rbf) &     0.462 &     0.538 &     0.615 \\
                & coGOL (rbf) &     0.385 &     0.423 &     0.615 \\
\cline{1-5}
\multirow{3}{*}{squash-unstored} & OL (rbf) &     0.308 &     0.308 &     0.692 \\
                & GOL (rbf) &     0.308 &     0.308 &     0.692 \\
                & coGOL (rbf) &     0.308 &     0.308 &     0.692 \\
\cline{1-5}
\multirow{3}{*}{tae} & OL (rbf) &     0.553 &     0.724 &     0.500 \\
                & GOL (rbf) &     0.579 &     0.776 &     0.513 \\
                & coGOL (rbf) &     0.566 &     0.776 &     0.526 \\
\cline{1-5}
\multirow{3}{*}{toy} & OL (rbf) &     0.020 &     0.020 &     0.980 \\
                & GOL (rbf) &     0.053 &     0.053 &     0.947 \\
                & coGOL (rbf) &     0.040 &     0.040 &     0.960 \\
\cline{1-5}
\multirow{3}{*}{winequality-red} & OL (rbf) &     0.435 &     0.540 &     0.611 \\
                & GOL (rbf) &     0.446 &     0.556 &     0.605 \\
                & coGOL (rbf) &     0.433 &     0.524 &     0.608 \\
\bottomrule
\end{tabular}

